A Software Tool for Legal Drafting

Although many attempts at automated aids for legal drafting have been made, they were based on the construction of a new tool, completely from scratch. This is at least curious, considering that a strong parallelism can be established between a normative document and a software specification: both describe what an entity should or should not do, can or cannot do. In this article we compare normative documents and software specifications to find out their similarities and differences. The comparison shows that there are distinctive particularities, but they are restricted to a very specific subclass of normative propositions. The rest, we postulate, can be dealt with software tools. For such an enterprise the \FormaLex tool set was devised: an LTL-based language and companion tools that utilize model checking to find out normative incoherences in regulations, contracts and other legal documents. A feature-rich case study is analyzed with the presented tools.

==> eptcsdata.tex <==
\providecommand{\firstpage}{71}
\providecommand{\publicationstatus}{E. Pimentel, V. Valero (Eds.): Workshop on Formal Languages\\
and Analysis of Contract-Oriented Software 2011 (FLACOS'11)\\
EPTCS 68, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.68.7}{10.4204/EPTCS.68.7}}

